BRICS: Bi-level feature Representation of Image CollectionS

We present BRICS, a bi-level feature representation for image collections, which consists of a key code space on top of a feature grid space. Specifically, our representation is learned by an autoencoder to encode images into continuous key codes, which are used to retrieve features from groups of multi-resolution feature grids. Our key codes and feature grids are jointly trained continuously with well-defined gradient flows, leading to high usage rates of the feature grids and improved generative modeling compared to discrete Vector Quantization (VQ). Differently from existing continuous representations such as KL-regularized latent codes, our key codes are strictly bounded in scale and variance. Overall, feature encoding by BRICS is compact, efficient to train, and enables generative modeling over key codes using the diffusion model. Experimental results show that our method achieves comparable reconstruction results to VQ while having a smaller and more efficient decoder network (50% fewer GFlops). By applying the diffusion model over our key code space, we achieve state-of-the-art performance on image synthesis on the FFHQ and LSUN-Church (29% lower than LDM, 32% lower than StyleGAN2, 44% lower than Projected GAN on CLIP-FID) datasets.

==> backup.tex <==
%Compared to VQ-reg, KL-reg tends to encourage the latent space to be smooth and densely packed, which can result in the loss of fine-grained details and variations in the generated samples. This can be problematic when modeling complex and diverse datasets where preserving such details is crucial.
% in the neighborhoods modeled by Gaussian distribution

%To apply diffusion model on ordinary 8-bit images, it has been shown that setting the basic channel size of UNet as 64 or 128 can achieve satisfactory generation quality~\cite{ho2020denoising,song2020score,saharia2022photorealistic}. 
%When doing denoising diffusion on the indices of codebook entries, latent diffusion models \cite{rombach2022high} adopted a larger basic channel size of 256. For 8-bit images, the numerical precision is $\frac{1}{256}$. For the indices of codebook entries, the numerical precision is determined by the size of VQ codebook, i.e., if the codebook size is 1024, the precision will be $\frac{1}{1024}$. Based on this observation, we assume the numerical precision of the data determines the network size of UNets performing denoising (a finer precision requires a larger network size). Using the limited capacity of UNet and limited steps of denoising processes to precisely generate data in continuous values would be challenging.  
%However, intuitively, a finer precision requires a larger network size. Using the limited capacity of UNet and limited steps of denoising processes to precisely generate data in continuous values would be challenging.

%and ignores their connection with the hash tables.
%We take a different approach against VQ-Reg and KL-Reg, based on the connections between key codes with hash tables.

%the inherent discrete components in our framework.
%In the hash tables, we define discrete resolutions in each level. For each resolution, we find adjacent grid nodes around a unit continuous indexing $z_{i,j}^s$ and do linear interpolations between the values of these nodes\cite{muller2022instant}. 


\textbf{Relaxed data precision.} 
\yz{To apply our method in the task of image synthesis, we perform latent diffusion~\cite{rombach2022high}, one of the state-of-the-art generative methods, upon our key code representation. (needs some papers to verify this claim:) Diffusion process typically favors data with low precision representationm, such as the RGB values~\cite{dhariwal2021diffusion}, to generate quality data.
However, the vanilla latent codes are typically in high precision. To ease the training process, LDM~\cite{rombach2022high} proposed to use (1) VQ-Reg which quantizes the latent into the indices of codebook entries or (2) KL-Reg which encourages the learned distribution in the latent space to match a predefined target distribution, with the same goal to lower data precision. 
}

\yz{
We prefer not to establish another codebook for our key codes, which will bring extra storage cost in addition to hash tables.}
\textcolor{red}{Here need some reason why we do not use KL-Reg, one option is that KL-Reg usually result in the loss of fine-grained details and variations in the generated samples.}
\yz{
The connection between our key code and hash table inspired the development of a novel method for data precision control.}
We illustrate this relaxed precision mechanism in a simplified 1D grid of the finest resolution. As shown in \autoref{fig:controlled_procesion}, we inject a noise $\epsilon_o \sim \mathcal{N}(0, \frac{1}{(4r_{max})^2})$ to $z_{i,j}^s$ 
 during autoencoding training. 
 \yz{After training, the autoencoder will learn to produce sharp reconstruction results from perturbed key codes as long as they are within the interval of $z_{i,j}^s \pm \frac{1}{2r_{max}}$, which we call it a relaxed precision.
 As a result, the denoised key codes after denoising process do not necessarily need to be very precise to produce good results.}
 

==> tables/kl_reg_vs_relaxed_precision_reconstruction.tex <==
\begin{table}[h]
\centering
\resizebox{0.48\textwidth}{!}{
\tiny
\begin{tabular}{ccccc}
     \thickhline
     \addlinespace[2pt] 
     Method                                 &  Code Size & LPIPS$\downarrow$ & SSIM $\uparrow$ & PSNR $\uparrow$ \\ \hline
     \addlinespace[2pt] 
     \hline
     \addlinespace[2pt]
     Ours ($\epsilon_0$)                       &$64\times 64 \times 4$ & 0.035$\pm$0.029 & 0.85$\pm$0.13 & 26.53$\pm$7.24 \\
     Ours (KL-reg)                      &$64\times 64 \times 4$ & \textbf{0.036$\pm$0.030} & \textbf{0.84$\pm$0.13} & \textbf{26.45$\pm$7.25} \\
     \addlinespace[2pt]
     \thickhline
\end{tabular}}
 \vspace{4pt}
 \caption{Reconstruction metrics of ours relaxed precision setting vs the KL-reg on the $\hat{z}_{i,j}^s$, evaluated on the validation split of LSUN-Church dataset~\cite{yu2015lsun} after training on 2400K images.}
  \label{tab:ours_vs_kl_recon}

\end{table}

